SpeechCLIP+: Self-supervised multi-task representation learning for speech via CLIP and speech-image data

The recently proposed visually grounded speech model SpeechCLIP is an innovative framework that bridges speech and text through images via CLIP without relying on text transcription. On this basis, this paper introduces two extensions to SpeechCLIP. First, we apply the Continuous Integrate-and-Fire (CIF) module to replace a fixed number of CLS tokens in the cascaded architecture. Second, we propose a new hybrid architecture that merges the cascaded and parallel architectures of SpeechCLIP into a multi-task learning framework. Our experimental evaluation is performed on the Flickr8k and SpokenCOCO datasets. The results show that in the speech keyword extraction task, the CIF-based cascaded SpeechCLIP model outperforms the previous cascaded SpeechCLIP model using a fixed number of CLS tokens. Furthermore, through our hybrid architecture, cascaded task learning boosts the performance of the parallel branch in image-speech retrieval tasks.

==> method_v1.tex <==
%In this section, we introduce three architectures of SpeechCLIP+: parallel SpeechCLIP+, cascaded SpeechCLIP+ and hybrid SpeechCLIP+. During training, the input to the model is a batch of paired images and audio waveforms. Images are passed to CLIP's image encoder to extract image representations, and audio waveforms are passed to a pre-trained speech encoder and an additional transformer encoder to extract audio representations. CLIP's text and image encoders are frozen during SpeechCLIP+ training. They serve as projectors of the pre-trained image-text semantic space. Unlike SpeechCLIP, we fine-tune the pre-trained speech encoder and take the last hidden state of it, instead of the weighted sum of all hidden states. Moreover, we adopt WavLM Base+~\cite{chen2022wavlm} instead of HuBERT~\cite{hsu2021hubert} because WavLM Base+ is pre-trained on a more diverse dataset and may provide a better initialization for downstream tasks~\cite{yang2021superb}. The loss function is the masked version of the decoupled contrastive loss~\cite{yeh2022decoupled}, which is computed from audio and image representations and tailored for the case where an image has multiple associated spoken captions. 

During SpeechCLIP (either cascaded or parallel) training, the input to the model is a batch of paired images and audio waveforms. Images are passed to CLIP's image encoder to extract image representations, and audio waveforms are passed to a pre-trained SSL speech encoder (i.e., HuBERT~\cite{hsu2021hubert}) to extract audio representations, as shown in~\ref{fig:hybrid_overview}. CLIP's text and image encoders are frozen during SpeechCLIP training. They serve as projectors of the pre-trained image-text semantic space. The loss function is the masked version of the decoupled contrastive loss~\cite{yeh2022decoupled}, which is computed from audio and image representations and tailored for the case where an image has multiple associated spoken captions. Given a batch of paired audio and image representations $\{A_i,I_i\}_{i=1}^B$, the loss function $\mathcal{L}$ is defined as 
\begin{equation}
\label{eq:masked_cl}
\mathcal{L} = \frac{\mathcal{L}_{A \to I} + \mathcal{L}_{I \to A}}{2},
\end{equation}
where
\begin{equation}
\label{eq:masked_c2}
\begin{aligned}
    \mathcal{L}_{A \to I} &= -\dfrac{1}{B}\sum_{i=1}^{B}\log\dfrac{\sum_{j=1}^{B}M_{ij}e^{{\cos(A_i, I_j)}/{\tau}}}{\sum_{j=1}^{B}(1-M_{ij})e^{{\cos(A_i, I_j)}/{\tau}}} \\
    \mathcal{L}_{I \to A} &= -\dfrac{1}{B}\sum_{j=1}^{B}\log\dfrac{\sum_{i=1}^{B}M_{ij}e^{{\cos(A_i, I_j)}/{\tau}}}{\sum_{i=1}^{B}(1-M_{ij})e^{{\cos(A_i, I_j)}/{\tau}}}.
\end{aligned}
\end{equation}
$\tau\in\mathbb{R}_{>0}$ is a tunable hyper-parameter. $M_{ij}$ is an indicator that is $1$ if $A_i$ and $I_j$ are semantically related pairs, and $0$ otherwise.

%\subsection{Parallel SpeechCLIP+}
%For parallel SpeechCLIP+ (parallel+), as with parallel SpeechCLIP~\cite{shih2022speechclip}, we simulate CLIP training by aligning images to their associated spoken captions. We concatenate a learnable CLS token at the beginning of the SSL audio features, pass the sequence through the transformer encoder, and use the CLS representation to compute the loss using Eqs. (\ref{eq:masked_cl}) and (\ref{eq:masked_c2}).

\subsection{Cascaded SpeechCLIP+}
As shown in Fig. \ref{fig:SpeechCLIP}, in cascaded SpeechCLIP, the transformer encoder is cascaded with the CLIP text encoder to force it to extract semantic information from sub-word level content. $K$ learnable CLS tokens (the best $K$ is 8 in~\cite{shih2022speechclip}) are added at the beginning of the SSL audio features, and the whole sequence is passed through the transformer encoder. The output CLS tokens are then batch-normalized to match the mean and variance of CLIP's Byte-Pair Encoding (BPE) token embeddings and vector-quantized into BPE tokens, which are then fed into the CLIP text encoder to generate representations. These representations are used to compute the loss using Eqs. (\ref{eq:masked_cl}) and (\ref{eq:masked_c2}).

As shown in Fig. \ref{fig:SpeechCLIP+}, in cascaded SpeechCLIP+, instead of extracting keyword information through a fixed number of learnable CLS tokens, we apply the Continuous Integrate-and-Fire (CIF) mechanism~\cite{dong2020cif} to segment frame-level features into a subword-level keyword sequence. CIF is a soft and monotonic alignment to segment the input features with a given weight, which scales the amount of information contained in each feature. We set the target length of the CIF to \textcolor{red}{5\%} of the input length, based on the average ratio between the length of the BPE-text token sequence and the output feature length of HuBERT, as observed during our experimentation. This approach allows for a variable number of keywords, which is proportional to the output length of the transformer encoder. After the CIF mechanism, same as cascaded SpeechCLIP, we employ batch normalization and vector quantization to generate BPE tokens. These tokens are then input into the CLIP text encoder to extract representations, which are subsequently used to compute the loss $\mathcal{L}_c$ using Eqs. (\ref{eq:masked_cl}) and (\ref{eq:masked_c2}).
%Note that this is a crucial process for effective training~\cite{shih2022speechclip}.

\subsection{Hybrid SpeechCLIP}
Two types of SpeechCLIP~\cite{shih2022speechclip} are expected to benefit speech encoders from semantically related images through different alignment methods. Parallel SpeechCLIP enables speech encoders to benefit from utterance summarization, while cascaded SpeechCLIP enables speech encoders to benefit from capturing subword-level information from utterances.  The advantages of combining the two approaches are quite intuitive. As shown in Fig. \ref{fig:SpeechCLIP+}, in hybrid SpeechCLIP, the parallel branch and the cascaded branch are trained jointly. 
%Furthermore, the inflexibility of the fixed number of keywords in the cascaded SpeechCLIP design limits its applicability. As shown in Fig. \ref{fig:model_arch}, we design a new architecture called hybrid SpeechCLIP+ (hybrid+) to integrate the strengths of both architectures and be able to output a variable number of keywords.

%Imitating the design of the corresponding SpeechCLIP, we design two branches, a parallel branch and a cascaded branch, and calculate their contrastive losses respectively. Similar to SpeechCLIP, we also add a learnable CLS token at the beginning of the audio features and pass the whole sequence through the transformer encoder's layers. Then, the representations will be sent to different branches to compute the contrastive loss separately.


\subsubsection{Parallel branch}
The parallel branch is the same as parallel SpeechCLIP. The first representation (CLS) of the transformer encoder's output is used to compute the loss $\mathcal{L}_p$ using Eqs. (\ref{eq:masked_cl}) and (\ref{eq:masked_c2}).

\subsubsection{Cascaded branch}
The cascaded branch can be either cascaded SpeechCLIP or cascaded SpeechCLIP+. 
%The remaining representations of the transformer encoder's output corresponding to the SSL acoustic features are passed to the cascaded branch. Following cascaded SpeechCLIP, we cascade the transformer encoder with CLIP's text encoder, forcing it to capture semantic information of the keywords in the given utterance. However, we do not extract keyword information through a fixed number of learnable CLS tokens but apply the continuous integrate-and-fire (CIF) mechanism~\cite{dong2020cif} to segment frame-level features into a subword-level keyword sequence. CIF is a soft and monotonic alignment to segment the input features with a given weight, which scales the amount of information contained in each feature. We set the target length of the CIF to 5\% of the input length, based on the average ratio between the length of the BPE-text token sequence and the output feature length of WavLM, as observed during our experimentation. This approach allows for a variable number of keywords, which is proportional to the output length of the transformer encoder. After the CIF mechanism, same as cascaded SpeechCLIP, we employ batch normalization and vector quantization to generate quantized keywords. These quantized keywords are then input into CLIP's text encoder to extract representations, which are subsequently used to compute the loss $\mathcal{L}_c$ using Eqs. (\ref{eq:masked_cl}) and (\ref{eq:masked_c2}).

\subsubsection{Training loss}
The training loss $\mathcal{L}$ of hybrid SpeechCLIP is a combination of $\mathcal{L}_p$ and $\mathcal{L}_c$: 
\begin{equation}
\mathcal{L} = \lambda^p\mathcal{L}_p + \lambda^c\mathcal{L}_c,
\end{equation}
where $\lambda^p$ and $\lambda^c$ are tunable hyper-parameters.

%In the next section, we conduct several experiments, keyword extraction, spoken bag-of-words prediction and ZeroSpeech2021 semantics to examine models' representations.

%In this section, we introduce three architectures of SpeechCLIP+: parallel SpeechCLIP+, cascaded SpeechCLIP+ and hybrid SpeechCLIP+. During training, the input to the model is a batch of paired images and audio waveforms. Images are passed to CLIP's image encoder to extract image representations, and audio waveforms are passed to a pre-trained speech encoder and an additional transformer encoder to extract audio representations. CLIP's text and image encoders are frozen during SpeechCLIP+ training. They serve as projectors of the pre-trained image-text semantic space. Unlike SpeechCLIP, we fine-tune the pre-trained speech encoder and take the last hidden state of it, instead of the weighted sum of all hidden states. Moreover, we adopt WavLM Base+~\cite{chen2022wavlm} instead of HuBERT~\cite{hsu2021hubert} because WavLM Base+ is pre-trained on a more diverse dataset and may provide a better initialization for downstream tasks~\cite{yang2021superb}. The loss function is the masked version of the decoupled contrastive loss~\cite{yeh2022decoupled}, which is computed from audio and image representations and tailored for the case where an image has multiple associated spoken captions. 

During SpeechCLIP (either cascaded or parallel) training, the input to the model is a batch of paired images and audio waveforms. Images are passed to CLIP's image encoder to extract image representations, and audio waveforms are passed to a pre-trained SSL speech encoder (i.e., HuBERT~\cite{hsu2021hubert}) to extract audio representations. CLIP's text and image encoders are frozen during SpeechCLIP training. They serve as projectors of the pre-trained image-text semantic space. The loss function is the masked version of the decoupled contrastive loss~\cite{yeh2022decoupled}, which is computed from audio and image representations and tailored for the case where an image has multiple associated spoken captions. Given a batch of paired audio and image representations $\{A_i,I_i\}_{i=1}^B$, the loss function $\mathcal{L}$ is defined as 
\begin{equation}
\label{eq:masked_cl}
\mathcal{L} = \frac{\mathcal{L}_{A \to I} + \mathcal{L}_{I \to A}}{2},
\end{equation}
where
\begin{equation}
\label{eq:masked_c2}
\begin{aligned}
    \mathcal{L}_{A \to I} &= -\dfrac{1}{B}\sum_{i=1}^{B}\log\dfrac{\sum_{j=1}^{B}M_{ij}e^{{\cos(A_i, I_j)}/{\tau}}}{\sum_{j=1}^{B}(1-M_{ij})e^{{\cos(A_i, I_j)}/{\tau}}} \\
    \mathcal{L}_{I \to A} &= -\dfrac{1}{B}\sum_{j=1}^{B}\log\dfrac{\sum_{i=1}^{B}M_{ij}e^{{\cos(A_i, I_j)}/{\tau}}}{\sum_{i=1}^{B}(1-M_{ij})e^{{\cos(A_i, I_j)}/{\tau}}}.
\end{aligned}
\end{equation}
$\tau\in\mathbb{R}_{>0}$ is a tunable hyper-parameter. $M_{ij}$ is an indicator that is $1$ if $A_i$ and $I_j$ are semantically related pairs, and $0$ otherwise.

%\subsection{Parallel SpeechCLIP+}
%For parallel SpeechCLIP+ (parallel+), as with parallel SpeechCLIP~\cite{shih2022speechclip}, we simulate CLIP training by aligning images to their associated spoken captions. We concatenate a learnable CLS token at the beginning of the SSL audio features, pass the sequence through the transformer encoder, and use the CLS representation to compute the loss using Eqs. (\ref{eq:masked_cl}) and (\ref{eq:masked_c2}).

\subsection{Cascaded SpeechCLIP+}
As shown in Fig. \ref{fig:SpeechCLIP}, in cascaded SpeechCLIP, the transformer encoder is cascaded with the CLIP text encoder to force it to extract semantic information from sub-word level content. $K$ learnable CLS tokens (the best $K$ is 8 in~\cite{shih2022speechclip}) are added at the beginning of the SSL audio features, and the whole sequence is passed through the transformer encoder. The output CLS tokens are then batch-normalized to match the mean and variance of CLIP's Byte-Pair Encoding (BPE) token embeddings and vector-quantized into BPE tokens, which are then fed into the CLIP text encoder to generate representations. These representations are used to compute the loss using Eqs. (\ref{eq:masked_cl}) and (\ref{eq:masked_c2}).

As shown in Fig. \ref{fig:SpeechCLIP+}, in cascaded SpeechCLIP+, instead of extracting keyword information through a fixed number of learnable CLS tokens, we apply the Continuous Integrate-and-Fire (CIF) mechanism~\cite{dong2020cif} to segment frame-level features into a subword-level keyword sequence. CIF is a soft and monotonic alignment to segment the input features with a given weight, which scales the amount of information contained in each feature. We set the target length of the CIF to \textcolor{red}{5\%} of the input length, based on the average ratio between the length of the BPE-text token sequence and the output feature length of HuBERT, as observed during our experimentation. This approach allows for a variable number of keywords, which is proportional to the output length of the transformer encoder. After the CIF mechanism, same as cascaded SpeechCLIP, we employ batch normalization and vector quantization to generate BPE tokens. These tokens are then input into the CLIP text encoder to extract representations, which are subsequently used to compute the loss $\mathcal{L}_c$ using Eqs. (\ref{eq:masked_cl}) and (\ref{eq:masked_c2}).
%Note that this is a crucial process for effective training~\cite{shih2022speechclip}.

\subsection{Hybrid SpeechCLIP}
Two types of SpeechCLIP~\cite{shih2022speechclip} are expected to benefit speech encoders from semantically related images through different alignment methods. Parallel SpeechCLIP enables speech encoders to benefit from utterance summarization, while cascaded SpeechCLIP enables speech encoders to benefit from capturing subword-level information from utterances.  The advantages of combining the two approaches are quite intuitive. As shown in Fig. \ref{fig:SpeechCLIP+}, in hybrid SpeechCLIP, the parallel branch and the cascaded branch are trained jointly. 
%Furthermore, the inflexibility of the fixed number of keywords in the cascaded SpeechCLIP design limits its applicability. As shown in Fig. \ref{fig:model_arch}, we design a new architecture called hybrid SpeechCLIP+ (hybrid+) to integrate the strengths of both architectures and be able to output a variable number of keywords.

%Imitating the design of the corresponding SpeechCLIP, we design two branches, a parallel branch and a cascaded branch, and calculate their contrastive losses respectively. Similar to SpeechCLIP, we also add a learnable CLS token at the beginning of the audio features and pass the whole sequence through the transformer encoder's layers. Then, the representations will be sent to different branches to compute the contrastive loss separately.


\subsubsection{Parallel branch}
The parallel branch is the same as parallel SpeechCLIP. The first representation (CLS) of the transformer encoder's output is used to compute the loss $\mathcal{L}_p$ using Eqs. (\ref{eq:masked_cl}) and (\ref{eq:masked_c2}).

\subsubsection{Cascaded branch}
The cascaded branch can be either cascaded SpeechCLIP or cascaded SpeechCLIP+. 
%The remaining representations of the transformer encoder's output corresponding to the SSL acoustic features are passed to the cascaded branch. Following cascaded SpeechCLIP, we cascade the transformer encoder with CLIP's text encoder, forcing it to capture semantic information of the keywords in the given utterance. However, we do not extract keyword information through a fixed number of learnable CLS tokens but apply the continuous integrate-and-fire (CIF) mechanism~\cite{dong2020cif} to segment frame-level features into a subword-level keyword sequence. CIF is a soft and monotonic alignment to segment the input features with a given weight, which scales the amount of information contained in each feature. We set the target length of the CIF to 5\% of the input length, based on the average ratio between the length of the BPE-text token sequence and the output feature length of WavLM, as observed during our experimentation. This approach allows for a variable number of keywords, which is proportional to the output length of the transformer encoder. After the CIF mechanism, same as cascaded SpeechCLIP, we employ batch normalization and vector quantization to generate quantized keywords. These quantized keywords are then input into CLIP's text encoder to extract representations, which are subsequently used to compute the loss $\mathcal{L}_c$ using Eqs. (\ref{eq:masked_cl}) and (\ref{eq:masked_c2}).

\subsubsection{Training loss}
The training loss $\mathcal{L}$ of hybrid SpeechCLIP is a combination of $\mathcal{L}_p$ and $\mathcal{L}_c$: 
\begin{equation}
\mathcal{L} = \lambda^p\mathcal{L}_p + \lambda^c\mathcal{L}_c,
\end{equation}
where $\lambda^p$ and $\lambda^c$ are tunable hyper-parameters.

%In the next section, we conduct several experiments, keyword extraction, spoken bag-of-words prediction and ZeroSpeech2021 semantics to examine models' representations.

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{fig/climb.png}
    \vspace{-0.1cm}
    \caption{An example of keywords extracted by Cascaded SpeechCLIP+ from the Flickr8k dev set, showing the image, spoken caption, and extracted keywords with corresponding segments.}
    \label{fig:keywords}
    \vspace*{-10pt}
\end{figure*}

%\begin{figure*}
%    \centering
%    \includegraphics[width=0.9\textwidth]{fig/keywords_1.png}\\
%    \includegraphics[width=0.9\textwidth]{fig/keywords_2.png}
%    \vspace{-0.1cm}
%    \caption{Two examples of hybrid SpeechCLIP+'s extracting keywords from the Flickr8k dev set, each showing the image, spoken caption, and extracted keywords, along with corresponding segmentations.}
%    \label{fig:keywords}
%    \vspace*{-10pt}
%\end{figure*}


%\begin{figure*}
%    \centering
%    \includegraphics[width=0.9\textwidth]{fig/keywords_1.png}\\
%    \includegraphics[width=0.9\textwidth]{fig/keywords_2.png}
%    \vspace{-0.1cm}
%    \caption{Two examples of hybrid SpeechCLIP+'s extracting keywords from the Flickr8k dev set, each showing the image, spoken caption, and extracted keywords, along with corresponding segmentations.}
%    \label{fig:keywords}
%    \vspace*{-10pt}
%\end{figure*}

==> old/old_contents.tex <==
\section{OLD Experiments and Results}

 \begin{table}[th]
  \small
  \caption{Performance of keyword extraction in cosine semantics. For random, we randomly selected tokens as keywords to compute the score.}
%For each dataset, the models were trained on the train set and evaluated on the dev set.
  \label{tab:cos_sem}
  \centering
  \small
%  \begin{tabular}{l@{~}c@{~}}
%    \toprule
%    Model & Avg.\\
%    \midrule
%    & Flickr8k\\
%    \cmidrule{2-2}
%    Random & 0.055 \\
%    Cascaded+ & 0.129 \\
%    Hybrid+ & 0.126 \\
%    Cascaded~\cite{shih2022speechclip} & 0.181\\
%    \midrule
%    & SpokenCOCO\\
%    \cmidrule{2-2}
%    Random & 0.053 \\
%    Cascaded+ & 0.103 \\
%    Hybrid+ & 0.159 \\
%    Cascaded Large~\cite{shih2022speechclip} & \textbf{0.292}\\
%    \bottomrule
%  \end{tabular}
  \vspace*{-5pt}
  \begin{tabular}{l@{~~}c@{~~}c@{~~~}}
    \toprule
    Model & Flickr8k & SpokenCOCO\\
    \midrule
    Random & 0.055 & 0.053 \\
    Cascaded+ & 0.129 & 0.103 \\
    Hybrid+ & 0.126 & 0.159 \\
    Cascaded~\cite{shih2022speechclip} & 0.181 & -\\
    Cascaded Large~\cite{shih2022speechclip} & \textbf{0.289} & \textbf{0.292}\\
    \bottomrule
  \end{tabular}
  \vspace*{-10pt}
\end{table}

\subsection{Keyword extraction}
We evaluate hybrid+'s keyword extraction ability through qualitative and quantitative analyses. For qualitative analysis, from the examples from Flickr8k in Fig. \ref{fig:keywords}, we can observe hybrid+'s ability to capture semantically aligned keywords and their corresponding boundaries in the input speech, e.g., the extracted keyword ``DOGS'' corresponds to ``BLACK DOGS'' in the first example, and the extracted keywords ``JUMPING'' and ``GIRL'' correspond to ``JUMPING'' and ``GIRL'' in the second example. 

% Second, we discover some abstract keywords inferred by SpeechCLIP+. For instance, the first example's "CURLY", which might indicate the two black dogs' curling bodies while they're playing together.

For quantitative analysis, we do not adopt keyword hit rate~\cite{shih2022speechclip}, because this metric only considers keywords that hit the ground truth text caption, but ignores related keywords, such as ``GOOFY'' in Fig. \ref{fig:keywords}. To address this issue, we introduce a new metric called cosine semantics to evaluate how well output keywords align with text captions in the semantic space of CLIP's text embeddings. 
Given output keywords $\boldsymbol{k}=[k_1,k_2,\dots, k_m]$ ($k_p \neq k_q,\ \forall p, q$) and embeddings $\boldsymbol{t}=[t_1,t_2,\dots,t_n]$ of the corresponding text caption encoded by CLIP's text encoder, the cosine semantics of $\boldsymbol{k}$ is defined as
\begin{equation}
\dfrac{1}{m}\sum^{m}_{p=1} \max_{i \in \mathcal{S}} \cos(k_p, t_i),
\end{equation}
where $\mathcal{S} = \{i \mid t_i\text{ not yet aligned to any }k_q \in \boldsymbol{k}\}$ is used to not make different keywords align to the same word or word piece. 

The results are shown in Table \ref{tab:cos_sem}, where hybrid+ performs similarly to cascaded+ on FLickr8k, but performs better on the larger dataset SpokenCOCO. This implies that if we fine-tune the SSL speech encoder, the hybrid architecture can extract keywords with greater semantic meaning than the cascaded architecture, which may be attributed to the novel design of hybrid+, which can obtain semantic information not only from the subword level, but also from the utterance level. However, the performance of our models is lower than that of cascaded SpeechCLIP~\cite{shih2022speechclip}, which might suggest that frozen SSL speech encoders are better suited for keyword extraction tasks. 


% Lastly, we compute the average length and the variance of hybrid+'s outputting keyword sequence's length on datatset's dev set. For Flickr8k, the average length is 9.6 and variance is 11.6. On the other hand, the average length and the variance are 10.0 and 7.2 respectively for SpokenCOCO. The large variance implies that hybrid+ is outputting different numbers of keywords for different utterances.
% \begin{table}[th]
%   \caption{Average and the std of hybrid+'s outputting keyword sequence length on dataset's dev set}
%   \label{tab:kw_stat}
%   \centering
%   \begin{tabular}{lcc}
%     \toprule
%     & \multicolumn{2}{c}{Length}\\
%     Dataset & Avg. & Var.\\
%     \midrule
%     Flickr8k & 9.64 & 11.59\\
%     SC & 10.01 & 7.24\\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \subsection{Spoken bag-of-words prediction} 
% hybrid+'s ability to capture existing words as in Figure 2 is noteworthy, so following~\cite{kamper2017visually}, we consider the task of spoken bag-of-words (BoW) prediction to compare cascaded+ and hybrid+. This task is about given an utterance $X$, for each token $t$ in vocabulary, the model $f$ has to give a label $f_t(X) \in \{0, 1\}$ to determine whether the token exists in utterance. \jefftodo{}{Jeff: I've added the sentence below to claim that we can not compare with other works, does it sound reasonable? \textbf{"Note that our results cannot be compared to other works as we use quantized keywords for prediction and rely solely on pre-trained CLIP's bpe-tokens as vocabulary, while other works use word vocabulary."}}
% Moreover, since during the training stage we do not take the whole pre-trained CLIP bpe-tokens codebook to predict, but only the subset of tokens existing in the dataset, the predictable vocabulary size varies for different datasets (Flickr8 is about 8110, SC is about 19785). 
% We report the F1 score, recall and precision in table \ref{tab:BoW}. hybrid+ outperforms cascaded+ for all the metrics and all the datasets, which implies that the hybrid architecture is better than the cascaded architecture at discovering existing CLIP's bpe-tokens. 

% \begin{table}[th]
%   \caption{Spoken BoW prediction performance(\%). P, R and F denote precision, recall and F1 score respectively.}
%   \label{tab:BoW}
%   \centering
%   \begin{tabular}{l@{~~}c@{~~~}c@{~~}c@{~~}c@{~~}}
%     \toprule
%     Model & Dataset & P & R & F\\
%     \midrule
%     Cascaded+ & Flickr8k & 51.6 & 51.2 & 51.3\\
%     Hybrid+ & Flickr8k & 52.7 & 52.3 & 52.5\\
%     Cascaded~\cite{shih2022speechclip} & Flickr8k & 53.5 & 52.8 & 53.0\\
%     \midrule
%     Cascaded+ & SpokenCOCO & 52.0 & 51.5 & 51.3 \\
%     Hybrid+ & SpokenCOCO & 54.3 & 52.4 & 53.0\\
%     Cascaded Large~\cite{shih2022speechclip} & SpokenCOCO & 58.8 & &\\
%     \bottomrule
%   \end{tabular}
%   \vspace*{-10pt}
% \end{table}

\begin{table}[th]
  \small
  \caption{Performance on the ZeroSpeech 2021 semantics dev set. SC denotes SpokenCOCO, Lib and Syn denote LibriSpeech and synthetic speech, respectively, and h.b. denotes high budget, a benchmark for training models over 100 GPU hours.}
  \label{tab:z2021_dev}
  \centering
  \vspace*{-5pt}
  \begin{tabular}{ l@{~~}c@{~~~}c@{~~}c@{~~} }
    \toprule
    % & & \multicolumn{2}{c}{Semantic}\\
    % \cmidrule{3-4}
    Model & Training data & Lib & Syn\\
    \midrule
    WavLM Base+~\cite{chen2022wavlm} & MIX-94K & 14.06 & 2.48 \\
    VG Baseline (h.b.)~\cite{alishahi2021zr} & SC & 15.09 & 9.60 \\
    FaST-VGS+~\cite{peng2022fastvgsplus} & SC & 23.1 & 23.07 \\
    \midrule
    Cascaded+ & MIX-94K + Flickr8k & 15.38 & 9.98 \\
    Parallel+ & MIX-94K + Flickr8k & 18.45 & 9.10 \\
    Hybrid+ & MIX-94K + Flickr8k & 22.03 & 11.78 \\
    $\text{Cascaded}$~\cite{shih2022speechclip} & LS-960 + Flickr8k & 5.72 & -0.32\\
    $\text{Parallel}$~\cite{shih2022speechclip} & LS-960 + Flickr8k & 6.65 & -0.10\\
    \midrule
    Cascaded+ & MIX-94K + SC & 15.72 & 18.19 \\
    Parallel+ & MIX-94K + SC & \textbf{26.43} & \textbf{30.18} \\
    Hybrid+ & MIX-94K + SC & 10.11 & 13.20 \\
    $\text{Cascaded Large}$~\cite{shih2022speechclip} & LL-60k + SC & 15.01 & 3.96\\
    $\text{Parallel Large}$~\cite{shih2022speechclip} & LL-60k + SC & 10.67 & 7.30\\
    \bottomrule
  \end{tabular}
  \vspace*{-5pt}
\end{table}


\begin{table}[th]
  \small
  \caption{Performance on the ZeroSpeech 2021 semantics test set. parallel+ was trained on SpokenCOCO.}
  \label{tab:z2021_test}
  \centering
  \vspace*{-5pt}
  \begin{tabular}{ l@{~~}c@{~}c@{~}c@{~~}c@{~~} }
    \toprule
    % & \multicolumn{4}{c}{Semantic} \\
    % \cmidrule{2-5}
    & \multicolumn{2}{c}{Unweighted} & \multicolumn{2}{c}{Weighted}\\
    Model & Lib & Syn & Lib & Syn\\
    \midrule
    FaST-VGS+~\cite{peng2022fastvgsplus} & 14.32 & 15.1 & 12.78 & 17.99\\
    Parallel+ & \textbf{17.14} & \textbf{24.04} & \textbf{17.90} & \textbf{25.20} \\
    \midrule
    RoBERTa topline~\cite{alishahi2021zr} & 27.82 & 33.16 & 21.06 & 23.22\\
    \bottomrule
  \end{tabular}
  \vspace*{-12pt}
\end{table}

\subsection{ZeroSpeech2021 semantics}
We then evaluate SpeechCLIP+ on the ZeroSpeech2021 semantics task. This task is to assess how close the calculated similarity between spoken word pairs is to human similarity judgments using Spearman’s rank correlation coefficient. All models use cosine for similarity measure and mean pooling to temporally pool frame-based representations, except hybrid+ trained on SpokenCOCO, which uses maximum pooling. For each model, we choose the best result from all the layers of its SSL speech encoder and transformer encoder if the SSL speech encoder is fine tuned, and the best result from the layers of the transformer encoder otherwise. 
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth, trim={1.2cm 0cm 1.2cm 0.6cm},clip]{fig/z2021_semantics_syn.png}
    \vspace{-0.5cm}
    \caption{Layer-wise performance of WavLM Base+ and parallel+ evaluated on the ZeroSpeech2021 semantics dev-Syn set. \texttt{CNN} denotes the CNN feature extractor before the SSL speech encoder, and $\texttt{Trm}_i$ denotes the i-th layer of the additional transformer encoder.}
    \label{fig:z2021_layers}
    \vspace*{-5pt}
\end{figure}
\begin{table}[th]
  \small
  \caption{Performance of models with or without fine-tuning the SSL speech encoder evaluated on the ZeroSpeech2021 semantics dev set.}
  \label{tab:z2021_finetune}
  \vspace*{-5pt}
  \centering
  \begin{tabular}{ l@{~~}c@{~}c@{~}c@{~}c@{~} }
    \toprule
    % & & \multicolumn{2}{c}{Semantic}\\
    % \cmidrule{3-4}
    Model & Fine-tune & Lib & Syn\\
    \midrule
    Parallel+ & False & 6.19 & 8.28\\
    Parallel+ & True & \textbf{26.43} & \textbf{30.18}\\
    \midrule
    Cascaded+ & False & 3.29 & 3.25\\
    Cascaded+ & True & 15.72 & 18.19\\
    \bottomrule
  \end{tabular}
  \vspace*{-10pt}
\end{table}
From Table \ref{tab:z2021_dev}, we can see that parallel+ outperforms the previous state-of-the-art FaST-VGS+. Furthermore, the SpeechCLIP+ models trained on Flickr8k perform better on Lib than on Syn, while the SpeechCLIP+ models trained on SpokenCOCO perform better on Syn than on Lib. This suggests that the performance on LibriSpeech may be dominated by the large pre-trained dataset MIX-94K (94k hours of speech), which includes LibriLight, while the performance on synthetic speech can be substantially improved by the image-speech datasets Flickr8k (46 hours of speech) and SpokenCOCO (742 hours of speech). Table \ref{tab:z2021_dev} also shows that parallel+ models generally outperform cascaded+ models, suggesting that fine-tuning SSL models with summary information is better suited for this task than trying to capture subword-level information. Moreover, the poor performance of hybrid+ models may be due to the short length of some input audio, which contains only one spoken word, resulting in insufficient information to perform summary and subword-level information extraction from the input audio. From Table \ref{tab:z2021_dev}, we can also see that all SpeechCLIP+ models outperform their counterpart SpeechCLIP models~\cite{shih2022speechclip}. 

To investigate layer-wise performance, we show the performance of each encoder layer in parallel+ and WavLM Base+ evaluated on the ZeroSpeech 2021 semantics dev-Syn set in Fig. \ref{fig:z2021_layers}. We observe that the last layer of the additional transformer encoder yields the best performance, suggesting that the layers of the transformer encoder contain more semantic information. 

%However, as SpeechCLIP does not involve fine-tuning of the speech encoder, we avoided iterating through it to achieve the best scores, as it is the same as taking HuBERT~\cite{hsu2021hubert} to evaluate.

Lastly, we evaluate our best model parallel+ on the ZeroSpeech2021 semantics test set. 
The results are shown in Table \ref{tab:z2021_test}. We can see that parallel+ outperforms the previous state-of-the-art FaST-VGS+, and even surpasses the RoBERTa topline in the setting of weighted scores and synthetic speech.

\subsection{Ablation study of SpeechCLIP+'s extensions}
We investigate which extensions of SpeechCLIP+ contribute more to performance improvements.
%, including 1) fine-tuning the backbone SSL speech encoder, 2) using WavLM Base+ instead of HuBERT, and 3) using a hybrid model combining cascaded and parallel architectures.

%For studies 1 and 2, we train the models on SpokenCOCO and evaluate them on the ZeroSpeech2021 semantics dev set by selecting the best result from all layers. For the study of 3., although this paper is not primarily focused on image retrieval tasks, we evaluate our models for image-speech retrieval on Flickr8k, given their original training purpose. Furthermore, we compare our results with SpeechCLIP~\cite{shih2022speechclip} in this study.

\noindent\textbf{Fine-tuning SSL speech encoders.} We evaluate the effectiveness of fine tuning WavLM Base+. The models are trained on SpokenCOCO
and evaluated on the ZeroSpeech2021 semantics dev set. 
The results in Table \ref{tab:z2021_finetune} confirm the benefit of fine-tuning the SSL speech encoder, showing that for semantically related tasks, VGS can boost performance of the SSL speech encoder.
%For each model, we choose the best result from all the layers of its SSL speech encoder and transformer encoder if the SSL speech encoder is fine tuned, and the best result from the layers of the transformer encoder otherwise. 
%For those models whose SSL speech encoders are not fine-tuned, we follow ~\cite{shih2022speechclip} to take the weighted sum of all hidden states for training, and evaluate the non-frozen transformers' features. The results are shown in Table \ref{tab:z2021_finetune}, which manifests the improvements from fine-tuning the speech encoders, indicating that for higher-level, e.g., semantic related tasks, VGS can boost pre-trained speech encoder's performance.


\noindent\textbf{Impact of the backbone SSL model.} We compare the performance of models using WavLM Base+ and HuBERT SSL speech encoders. The models are trained on SpokenCOCO and evaluated on the ZeroSpeech2021 semantics dev set. The results in Table \ref{tab:z2021_backbone} indeed show that WavLM Base+ is more effective than HuBERT. The dramatic improvement on the Syn set may be attributed to the increased dataset diversity in MIX-94K, which allows WavLM Base+ to better adapt to synthesized speech with VGS training.

%Since we change the speech encoder in SpeechCLIP~\cite{shih2022speechclip} from HuBERT to WavLM Base+, Naturally we want to ask, how much improvement has been brought about by this change? The results are presented in Table \ref{tab:z2021_backbone}. 

\begin{table}[th]
  \small
  \caption{Performance of models with different backbone speech encoders evaluated on the ZeroSpeech2021 semantics dev set.}
  \label{tab:z2021_backbone}
  \vspace{-5pt}
  \centering
  \begin{tabular}{ l@{~~}c@{~~}c@{~}c@{~}c@{~}}
    \toprule
    % & & \multicolumn{2}{c}{Semantic}\\
    % \cmidrule{3-4}
    Model & Backbone & Lib & Syn\\
    \midrule
    Parallel+ & HuBERT & 24.78 & 20.49\\
    Parallel+ & WavLM Base+ & \textbf{26.43} & \textbf{30.18}\\
    \midrule
    Cascaded+ & HuBERT & 12.68 & 15.95\\
    Cascaded+ & WavLM Base+ & 15.72 & 18.19\\
    \bottomrule
  \end{tabular}
  \vspace{-10pt}
\end{table}
\begin{table}[th]
  \small
  \caption{Image-speech retrieval performance on Flickr8k. The superscript $*$ indicates that there is only cascaded branch in the model (similar to cascaded but with variable number of keywords), and the subscripts C and P indicate that the representation of cascaded or parallel branches is used for retrieval.}
  \label{tab:recall}
  \vspace*{-5pt}
  \centering
  \begin{tabular}{ l@{~~}c@{~~}c@{~~}c@{~~}c@{~}c@{~~}c@{~~}c@{~~} }
    \toprule
    & \multicolumn{3}{c}{Speech $\rightarrow$ Image} & & \multicolumn{3}{c}{Image $\rightarrow$ Speech}\\
    \cmidrule{2-4}
    \cmidrule{6-8}
    Model& R@1 & R@5 & R@10 & & R@1 & R@5 & R@10\\
    \midrule
    Parallel+& 24.2 & 55.2 & 69.9 & & 37.2 & 73.0 & 83.7\\ 
    Parallel~\cite{shih2022speechclip}&
    \textbf{26.7} & \textbf{57.1} & 70.0 & & \textbf{41.3} & \textbf{73.9} & \textbf{84.3}\\
    \midrule
    Cascaded+& 6.2 & 22.0 & 33.8 & & 7.3 & 26.3 & 40.5\\
    Cascaded~\cite{shih2022speechclip}& 8.2 & 25.7 & 37.2 & & 14.1 & 34.5 & 49.2\\
    \midrule
    $\text{Hybrid+}^{*}$& 0.4 & 1.7 & 3.2 & & 0.7 & 2.1 & 3.6\\
    $\text{Hybrid+}_\text{C}$& 3.5 & 13.1 & 21.1 & & 4.5 & 15.7 & 25\\
    $\text{Hybrid+}_\text{P}$& 24.1 & 56.4 & \textbf{70.1} & & 40.1 & 73.9 & 83.4\\
    \bottomrule
  \end{tabular}
  \vspace*{-10pt}
\end{table}
 
\noindent\textbf{Image-Speech retrieval.} We evaluate our models on the image-speech retrieval task using Flickr8k. The ``Speech $\rightarrow$ Image'' task is to retrieve the corresponding image given a spoken caption, and the ``Image $\rightarrow$ Speech'' task is to retrieve the corresponding spoken caption given an image. 
The results are shown in Table \ref{tab:recall}. 
The reason why the hybrid+ models did not achieve good results as expected may be due to the CIF mechanism, because we can see that hybrid+* is worse than Cascaded+, and the difference between the two is only in the use of a fixed number of keywords and a variable number of keywords obtained by CIF. Interestingly, hybrid+'s parallel branch outperforms parallel+, suggesting a mutual support between the parallel and cascaded branches in hybrid+. Our SpeechCLIP+ models were not able to outperform the state-of-the-art SpeechCLIP~\cite{shih2022speechclip} on the image-speech retrieval task, suggesting the need for further research and hyper-parameter tuning.
%Nonetheless, our paper's main focus does not center on this topic.

%The suggest that the hybrid+ model's performance suffers when trained only with the CIF mechanism, as evidenced by the inferior scores in the second row when compared to the first. This highlights the importance of the parallel branch in preventing retrieval failure.
% Lastly, we provide the layer-wise performance in figure \ref{fig:z2021_layers}. We can observe that first, WavLM Base+ performs surprisingly well on Lib., since WavLM Base+ is pre-trained on Mix 94k hr containing LibriLight\cite{kahn2020libri}; and second, parallel+'s last five layers have more semantic information, especially the last two transformer encoder layers.

\section{Conclusions}
In this paper, we attempt to boost the performance of pre-trained speech models on downstream tasks by leveraging visual content and other pre-trained modalities. On the ZeroSpeech2021 semantics task, SpeechCLIP+ outperforms SpeechCLIP~\cite{shih2022speechclip}, which confirms the advantage of our proposed extension. Our ablation study shows that expanding the diversity of pre-training data can provide better initialization for understanding the semantics of synthesized speech, while updating more pre-trained weights with visual information can greatly enhance the overall model's understanding of spoken word semantics. However, the framework still suffers from shortcomings, such as SpeechCLIP+ performing poorly compared to SpeechCLIP on downstream tasks of keyword extraction and image-speech retrieval. Furthermore, the poor performance of $\text{Hybord+}^{*}$ in Table \ref{tab:recall} may indicate that the CIF~\cite{dong2020cif} mechanism is not applicable without strong supervision, similar observations are also seen in ~\cite{meng2022compressing}. In our future work, we plan to add more guidance to CIF to enhance its ability to capture subword-level information.

\section{New experiment results}

\begin{table}[th]
  \small
  \caption{BPE extraction performance on Flickr8k.}
  \label{tab:BPE}
  \vspace*{-5pt}
  \centering
  \begin{tabular}{ l@{~~}c@{~~}c@{~~}c@{~~}c@{~}c@{~~}c@{~~}c@{~~} }
    \toprule
    & \multicolumn{3}{c}{w/o stop words} & & \multicolumn{3}{c}{w/ stop words}\\
    \cmidrule{2-4}
    \cmidrule{6-8}
    Model& R & P & F & & R & P & F\\
    \midrule
    Cascaded~\cite{shih2022speechclip}&
    7.39 & 0.94 & 1.66 & & 8.3  & 1.68 & 2.79\\
    Cascaded Large~\cite{shih2022speechclip}&
    5.27 & 0.75 & 1.31 & & 14.84 & 3.10 & 5.13\\
    \midrule
    Cascaded+& 27.16 & 3.55 & 6.29 & & 18.11 & 3.62 & 6.04\\
    Cascaded+ Large& \textbf{27.27} & \textbf{3.73} & \textbf{6.56} & & \textbf{20.74} & \textbf{4.2} & \textbf{6.99}\\
    \midrule
    Hybrid & 7.01 & 0.85 & 1.52 & & 5.41 & 1.06 & 1.77\\
    Hybrid Large & 6.73 & 0.86 & 1.53 & & 6.18 & 1.25 & 2.08\\
    \midrule
    Hybrid+ & 16.52 & 2.16 & 3.82 & & 11.40 & 2.23 & 3.73\\
    Hybrid+ Large & 21.69 & 2.92 & 5.15 & & 15.48 & 3.08 & 5.14\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[th]
  \small
  \caption{Whole word extraction performance on Flickr8k.}
  \label{tab:BPE}
  \vspace*{-5pt}
  \centering
  \begin{tabular}{ l@{~~}c@{~~}c@{~~}c@{~~}c@{~}c@{~~}c@{~~}c@{~~} }
    \toprule
    & \multicolumn{3}{c}{w/o stop words} & & \multicolumn{3}{c}{w/ stop words}\\
    \cmidrule{2-4}
    \cmidrule{6-8}
    Model& R & P & F & & R & P & F\\
    \midrule
    Cascaded+& \textbf{27.73} & 3.19 & 5.73 & & 18.31 & 3.33 & 5.63\\
    Cascaded+ Large& 27.59 &\textbf{3.20} & \textbf{5.74} & & \textbf{20.86} & \textbf{3.82} & \textbf{6.45}\\
    \midrule
    Hybrid+ & 17.30 & 1.93 & 3.48 & & 11.53 & 2.04 & 3.46\\
    Hybrid+ Large & 22.41 & 2.54 & 4.55 & & 15.56 & 2.79 & 4.73\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[th]
  \small
  \caption{Image-speech retrieval performance on Flickr8k.}
  \label{tab:IR}
  \vspace*{-5pt}
  \centering
  \begin{tabular}{ l@{~~}c@{~~}c@{~~}c@{~~}c@{~}c@{~~}c@{~~}c@{~~} }
    \toprule
    & \multicolumn{3}{c}{Speech $\rightarrow$ Image} & & \multicolumn{3}{c}{Image $\rightarrow$ Speech}\\
    \cmidrule{2-4}
    \cmidrule{6-8}
    Model& R@1 & R@5 & R@10 & & R@1 & R@5 & R@10\\
    \midrule
    Parallel~\cite{shih2022speechclip}&
    26.7 & 57.1 & 70.0 & & 41.3 & 73.9 & 84.3\\
    Parallel Large~\cite{shih2022speechclip}&
    39.1 & 72.0 & 83.0 & & 54.5 & 84.5 & 93.2\\
    \midrule
    Hybrid& 29.8 & 60.8 & 73.5 & & 40.9 & 71.6 & 83.9\\
    Hybrid+& 29.3 & 60.1 & 73.7 & & 39.7 & 72.8 & 83.4\\
    \midrule
    Hybrid Large& \textbf{43.1} & \textbf{75.6} & \textbf{85.2} & & \textbf{54.3} & 85.1 & 93.5\\
    Hybrid+ Large& 41.7 & 73.7 & 84.1 & & 54.2 & \textbf{86.8} & \textbf{94.2}\\
    \bottomrule
  \end{tabular}
\end{table}





\vfill\pagebreak

% References should be produced using the bibtex program from suitable
% BiBTeX files (here: strings, refs, manuals). The IEEEbib.bst bibliography
% style file from IEEE produces unsorted bibliography list.
% -------------------------------------------------------------------------
\bibliographystyle{IEEEbib}
\bibliography{strings,refs}
